Fair quantile regression

Quantile regression is a tool for learning conditional distributions. In this paper we study quantile regression in the setting where a protected attribute is unavailable when fitting the model. This can lead to "unfair'' quantile estimators for which the effective quantiles are very different for the subpopulations defined by the protected attribute. We propose a procedure for adjusting the estimator on a heldout sample where the protected attribute is available. The main result of the paper is an empirical process analysis showing that the adjustment leads to a fair estimator for which the target quantiles are brought into balance, in a statistical sense that we call $\sqrt{n}$-fairness. We illustrate the ideas and adjustment procedure on a dataset of 200,000 live births, where the objective is to characterize the dependence of the birth weights of the babies on demographic attributes of the birth mother; the protected attribute is the mother's race.

==> illustration.tex <==
\subsection{Birthweight Analysis}
\label{sec:birth}

%\begin{figure*}[ht]
%\begin{center}
%\def\pwidth{.15}
%\begin{tabular}{cccc}
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-1} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-2} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-3} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-16} \\
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-4} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-5} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-6} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-7} \\
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-8} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-9} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-10} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-11} \\
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-12} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-13} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-14} &
%\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-15}
%\end{tabular}
%\end{center}
%\caption{Quantile regression coefficients, including the protected
%  race variable $A$ (solid, salmon), and excluding $A$ (long dashed,
%  light blue). When the race variable $A$ is excluded, the variable ``married'' can be
% seen as serving as a kind of proxy.
% }
%\label{fig:all}
%\end{figure*}

\begin{figure*}[t]
\begin{center}
\def\pwidth{.16}
\begin{tabular}{ccccc}
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-1} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-2} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-3} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-14} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-16} \\
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-4} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-5} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-6} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-7} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-12} \\
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-8} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-9} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-10} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-11} &
\includegraphics[width=\pwidth\textwidth]{fig/qrcoeff-w-wo-black-13} \\
\end{tabular}
\end{center}
\caption{\small\it Quantile regression coefficients for the birth weight data. In each plot, the quantile $\tau$ runs along the horizontal axis, and the curves are the coefficients $\hat \beta_\tau$ for the variable noted on the vertical axis; the unit is grams. Solid/salmon coefficients are obtained when the race variable $A$ is included in the model, and dashed/blue coefficients are obtained when it is not included. When race is excluded, the strongly correlated variable ``married'' can be seen as serving as a kind of proxy.
 }
\label{fig:all}
\end{figure*}

The birth weight dataset from
\cite{abrevaya:01}, which is analyzed by
\cite{koenker2001quantile}, includes the weights
of 198,377 newborn babies, and other attributes of the babies
and their mothers, such as the baby's gender,
whether or not the mother is married, and the mother's age. One of the
attributes includes information about the race of the mother, which we treat as the
protected attribute $A$. The variable $A$ is binary---black ($A=1$) or
not black ($A=0$).

The birth weight is reported in grams. Education of the mother is divided
into four categories: less than high school, high school, some college
and college graduate. The default or omitted category is less than high school so
coefficients may be interpreted relative to this value. The
prenatal medical care of the mother is also divided into four
categories: no prenatal visit, and first prenatal
visit in the first, second or trimester of the pregnancy.
The omitted category is the group with a first visit in the
first trimester, making up almost 85 percent of the sample. An
indicator of whether the mother smoked during pregnancy is included in the model, as well
as mother's reported average number of cigarettes smoked per day. The
mother's reported weight gain during pregnancy (in pounds) is included
as a quadratic effect.

Figure~\ref{fig:all} shows the coefficients $\widehat{\beta}_\tau$ obtained
by fitting a linear quantile regression model, regressing birth weight
on all other attributes.  The model is fit two ways,
either including the protected
race variable $A$ (solid, salmon confidence bands), or excluding $A$ (long dashed,
light blue confidence bands).
The top-right figure shows that babies of black mothers weigh less on
average, especially near the lower quantiles where they weigh nearly
300 grams less compared to babies of nonblack mothers.  A description
of other aspects of this linear model is given by \cite{koenker2001quantile}.
For instance, the intercept of the model (upper left plot) may be
interpreted as ``the estimated conditional quantile function of the
birth weight distribution of a girl born to an unmarried, white mother
with less than a high school education, who is 27 years old and had a
weight gain of 30 pounds, didn't smoke, and had her first prenatal
visit in the first trimester of the pregnancy.''  A  striking aspect
of the plots is the disparity between birth weights of infants born to black and nonblack
mothers, especially at the left tail of the
distribution. In particular, at the 5th percentile of the conditional distribution,
the difference is more than 300 grams. Just as striking is the
observation that when the race attribute $A$ is excluded from the model, the variable
``married,'' with which it has a strong negative correlation, effectively serves
as a proxy, as seen by the upward shift in its regression
coefficients. However, this and the other variables do not completely
account for race, and as a result the model overestimates the weights
of infants born to black mothers, particularly at the lower
quantiles. For instance, at the target level $\tau=0.2$, the effective quantile for black mothers on a heldout set is $\hat\tau_1 \approx .29$. In other words, nearly 30\% of the births to black mothers have weights below the estimated level $\hat q_\tau(X)$, when the target is $20\%$. The target level of $20\%$ is more closely attained for the births to nonblack mothers, with $\hat\tau_0 \approx 0.184$.
We return to these data and analyses in Section~\ref{sec:experiments}, when we consider adjusting for race.

